ConEntail: An Entailment-based Framework for Universal Zero and Few Shot Classification with Supervised Contrastive Pretraining

A universal classification model aims to generalize to diverse classification tasks in both zero and few shot settings. A promising way toward universal classification is to cast heterogeneous data formats into a dataset-agnostic "meta-task" (e.g., textual entailment, question answering) then pretrain a model on the combined meta dataset. The existing work is either pretrained on specific subsets of classification tasks, or pretrained on both classification and generation data but the model could not fulfill its potential in universality and reliability. These also leave a massive amount of annotated data under-exploited. To fill these gaps, we propose ConEntail, a new framework for universal zero and few shot classification with supervised contrastive pretraining. Our unified meta-task for classification is based on nested entailment. It can be interpreted as "Does sentence a entails [sentence b entails label c]". This formulation enables us to make better use of 57 annotated classification datasets for supervised contrastive pretraining and universal evaluation. In this way, ConEntail helps the model (1) absorb knowledge from different datasets, and (2) gain consistent performance gain with more pretraining data. In experiments, we compare our model with discriminative and generative models pretrained on the same dataset. The results confirm that our framework effectively exploits existing annotated data and consistently outperforms baselines in both zero (9.4% average improvement) and few shot settings (3.5% average improvement).

==> deprecated_intro.tex <==
\section{Deprecated Intro}
% However, this setting is still far from the real-world use case. For example, as a cost of deprecating training data, $K \geq 8$ is required for \cite{xxx} to be fine-tuned in the test time; the prompt formulations of \cite{xxx} make the models unable to handle large $N$. 
% To address these issues, we propose a Universal Few-Shot Learning.
% \aysa{edited}


% \section{Deprecated Introduction}


  
% \begin{figure}[!hbt]
%     \centering
%     \includegraphics[width=\linewidth]{images/example.pdf}
%     \caption{A typical error made by local classifiers without global constraints.}
%     \label{fig:local_classifier_error}
% \end{figure}

% \begin{figure*}[!hbt]
%     \centering
%     \includegraphics[width=\linewidth]{images/overview.pdf}
%     \caption{An illustration of our end-to-end joint information extraction framework \textsc{OneIE} at the test stage.
%     We do not show all pairwise links for simplicity purposes.
%     }
%     \label{fig:overview}
% \end{figure*}

% directly related: pet -> semi-supervised training
% \haoran{we can have a "longer" intro for higher level and lower level motivations. lower level examples: a. Entailment as Few-Shot Learner sec3.1, b. Collecting Diverse Natural Language Inference Problems 
% for Sentence Representation Evaluation sec2. we may introduce exemplar theory in linguistics and explain the necessity of supervised contrastive learning there.}

% \haoran{1. I want to insert ``CDFSL task is doable only after LM-based universal classifier appeared'' into the introduction}

% \haoran{2. I think the long-existing few-shot learning paradigms in NLP is problematic. But it’s difficult to explain it in the introduction.}

% \haoran{3. My current example only shows the setting of “sentence classification with 2 parameters” and is not representative to all classification tasks.}



Pretrained Language Models (LMs) has bridged all the unlabeled data, from which they learned transferable context-aware embedding by self-supervised language model tasks\cite{???}.
Followed by fine-tuning on the training data annotated on a fixed label set, the LMs has achieved the state-of-the-art performance in a variety of downstream tasks \cite{???}.

  
\haoran{Cross Dataset Few Shot Learning is more than Cross Domain Cross Task Few Shot Learning.}
Recently, \cite{emmm} leverage label descriptions and propose unified frameworks for unlimited labels from different downstream tasks. They reformulate the targeted labels into proper prompts or cloze questions and reuse the LMs to complete the answer. These universal classifiers are especially effective in the low-resource setting. \citet{le2021many} have shown that the unified classifiers only need 1\% annotated data to achieve the same performance as the fully supervised learning. 
Comparing with the well-studied within-dataset few-shot learning \cite{fsl}, the newly evolved LM-based low-resourced learning is more challenging: 
(a) They are evaluated in multiple unseen datasets.
% while the K-Way-N-Shot focuses on one dataset. 
(b) They only have a few annotated data per label and no validation set for hyperparameter tuning.
% while the K-Way-N-Shot usually has large training and validation data to learn and to search hyperparamters. 
(c) They heavily rely on label-description-guided classification instead of exemplar comparison.
% Since train-test split of the new task in on dataset level instead of label level
Since the focus is on generalization across datasets, we refer it as \textbf{C}ross-\textbf{D}ataset \textbf{F}ew-\textbf{S}hot \textbf{L}earning (CDFSL). 




% The autoregressive LM, GPT-3, finds that different downstream tasks can be reformulated as cloze filling or label generationinto LMs thus enables direct inference in a unified framework with 0-32 examples as references.
% \cite{schick-schutze-2021-exploiting, schick-schutze-2021-just, gao2020making} builds the unified framework on Masked-Language-Model (MLM) to make parameter updating feasible. 
% EFL \cite{wang2021entailment} further extends the framework to model-agnostic method, to see whether or not the query sentence entails the label descriptions.

% \haoran{What problems do we solve? Learning to Segment Every Thing}


\begin{table*}[t]
\small
    \centering
    \begin{tabular}{l|p{0.6\columnwidth}|l|l|l}
    \toprule
               & Text & D(Q, (P, H)) & Entail & Label \\ \midrule
         $\text{Q}_a$  & [CLS] Foreign Bodies is an orchestral composition in three movements by the Finnish composer Esa-Pekka Salonen. \textbf{Alex Ross} of ``\textbf{The New Yorker}'' described the composition as "music of muscular, extroverted energy." [EOS] & & &  ? = employer of \\ \midrule
         $\text{P}_1$ & [CLS] \textbf{Linda J. Bilmes} (born 1960) is the Daniel Patrick Moynihan Senior Lecturer in Public Policy at \textbf{Harvard University}. [SEP] & \multirow{2}{*}{0.5} & \multirow{2}{*}{1} & \multirow{2}{*}{employer of}\\ 
        %  & & & &\\%\cline{2-2}
         $\text{H}_1$ & \textbf{Linda J. Bilmes} is the employer of \textbf{Harvard University}. [EOS]  & & \\ \midrule
         
         $\text{P}_2$ & [CLS] Her sister, \textbf{Kathryn Schulz} , is a staff writer for "\textbf{The New Yorker}". [SEP] & \multirow{2}{*}{0.9} & \multirow{2}{*}{1} & \multirow{2}{*}{employer of}\\ 
        %  & & & & \\ %\cline{2-2}
         $\text{H}_2$ & \textbf{Kathryn Schulz} is the employer of \textbf{The New Yorker}. [EOS]  & & \\ \midrule
         
         $\text{P}_3$ & [CLS] \textbf{I}’ve got good news for you: \textbf{the New Yorker} article in question is based on literally one guy on Twitter wanting to teach a shorter version of the case. It’s a completely manufactured fake controversy [SEP] & \multirow{2}{*}{-0.8} &\multirow{2}{*}{0} & \multirow{2}{*}{disagree with}\\ 
        %  & & & &\\ %\cline{2-2}
         $\text{H}_3$ & \textbf{I} disagree with \textbf{The New Yorker}. [EOS]  & & \\       
         \bottomrule
    \end{tabular}
    \caption{A universal classifier should be able to answer any question given only a label description and at least one example, even though the model may have never seen the same task.
    \haoran{My current example only shows the setting of “sentence classification with 2 parameters” and is not representative to all classification tasks}
    \haoran{Idea: some labels may also entail other labels, then we can use rules for precise data augmentation among different dataset.}}
    \label{tab:intro}
\end{table*}

% \haoran{the 700 sentences per label is problematic because they reuse them to simulate 5way-5shot FSL}

% \haoran{CDFSL task is doable only after LM-based universal classifier appeared}


% However, the existing few-shot learning datasets still does not fulfill the real-world requirement of the universal classifiers, because they focus on generalization of \textit{unseen labels from seen dataset} instead of \textit{labels from unseen datasets}.
% For example, FewRel \cite{emmm} annotates 100 relations x 700 sentences, then samples 64/100 relations for training and the remains for validation and testing. 
% By doing this, the models have access to 64 x 700 annotated data to learning the concept of relation extraction task.
% The sad truth is that for a new task, we usually have a simple annotation guideline, containing label descriptions and only 1-5 example sentences per label. 
% The generalization to labels across unseen datasets and the extremely low number of annotations create a minimum supervision scenario, which presents the new challenge of \textbf{C}ross-\textbf{D}ataset \textbf{F}ew-\textbf{S}hot \textbf{L}earning (CDFSL). 


Consider an extreme setting in CDFSL: suppose there is a new dataset with only an annotation guideline available. The models are expected to classify a large test set into 3 classes, each has a single labeled example in the guideline. Then the training data contains 3 sentences and is not sufficient for any existing models to fine-tune. 
% \aysa{the claim is too weak, please elaborate.}
% To solve this problem, we propose a contrastive one-shot learning method, which skip the task-specific fine-tuning and looks at the exemplar during the inference stage. 
To solve this problem, we propose a new method, which 
comprehends the label description with exemplar in the inference stage and 
learn the general label information from supervised intermediate training on all existing labeled dataset.
\aysa{how is this relevant to solving the problem? elaborate}
We bridge labeled data from different tasks by reformulating them into a unified \textbf{E}ntailment of \textbf{E}ntailment ($\text{E}^2$) task. 
\aysa{Why do you suddenly start talking about E2? How does it connect with the previous part?} 
For a query sentence $Q$, the model is asked whether or not $Q$ entails the exemplar entailment defined by the \text{label hypothesis} $H$ and its corresponding \text{premise} $P$.
For example, in Fig. \ref{tab:intro}, the model are asked to classify the query sentence $Q_a$ parametered by $Alex Ross$ and $The New Yorker$. The prediction is conducted by answering the question that whether $Q_a$ entails the exemplar entailment defined by $H_1$ and  $P_1$, both parametered by $LindaJ.Bilmes$ and $HarvardUniversity$.

The new method is good because ...

The experiment results are good ...



% The data utilization of our method includes three levels: 1. The off-the-shelf LMs pretrained on all unlabeled data. 2. The intermediate training of $\text{E}^2$ on labeled data from all available datasets. 3. The inference stage of $\text{E}^2$ on one or a few exemplar data from the new task of interest.
% The benefit of the separaiton 


% we integrate contrastive learining mechanism into supervised intermediate training, thus allow the model to look at the exemplar during inference stage.
% To solve this problem, we propose a supervised contrastive pretraining framework built on the off-the-shelf unsupervised LMs. 
% \haoran{not concise}
% Pretrained LMs are powerful as they learned from all unlabeled texts, from which the knowledge is transferable to most of downstream tasks. 
% Beyond unlabeled data, there are also decades of well-annotated data scattered in different tasks. We aim to make full use of all available labeled data in other tasks to help the model understand new tasks. 


% We materialize our motivation by reformulating all classification tasks into an entailment of entailment task.
% CDFSL task is challenging because 1) there is no large-scale annotated texts to learn dataset knowledge; 2) 
% The demand of few-shot learning is from the expensiveness of annotating data on \textbf{new} tasks, while there are large amount of \textbf{existing} datasets annotated by the NLP community for decades. 

% QCH(query=Sentence(tokens=['The', 'special', 'was', 'the', 'first', 'Muppets', '-', 'related', 'program', 'to', 'be', 'produced', 'with', 'ATV', 'and', 'ITC', ',', 'who', 'would', 'both', 'co', '-', 'produce', 'the', 'highly', 'successful', '"', 'The', 'Muppet', 'Show', '"', 'three', 'years', 'later', '.'], terms=['the', 'muppet', 'show', 'atv'], meta=None), context=Sentence(tokens=['Alex', 'Ross', 'of', '"', 'The', 'New', 'Yorker', '"', 'described', 'the', 'composition', 'as', '"', 'music', 'of', 'muscular', ',', 'extroverted', 'energy', '.', '"'], terms=['alex', 'ross', 'the', 'new', 'yorker'], meta=None), hypothesis=Sentence(tokens=['alex', 'ross', 'subject', 'employer', 'object', 'the', 'new', 'yorker'], terms=['alex', 'ross', 'the', 'new', 'yorker'], meta=None), blabel=None, mlabel='employer', meta=None)
% employer


% QCH(query=Sentence(tokens=['Josia', 'neblina', 'is', 'a', 'moth', 'of', 'the', 'family', 'Notodontidae', '.'], terms=['josia', 'notodontidae'], meta=None), context=Sentence(tokens=['Linda', 'J.', 'Bilmes', '(', 'born', '1960', ')', 'is', 'the', 'Daniel', 'Patrick', 'Moynihan', 'Senior', 'Lecturer', 'in', 'Public', 'Policy', 'at', 'Harvard', 'University', '.'], terms=['daniel', 'patrick', 'moynihan', 'harvard', 'university'], meta=None), hypothesis=Sentence(tokens=['daniel', 'patrick', 'moynihan', 'subject', 'employer', 'object', 'harvard', 'university'], terms=['daniel', 'patrick', 'moynihan', 'harvard', 'university'], meta=None), blabel=None, mlabel='employer', meta=None)
% employer



% And before you cry “fake news” Roger admitted that the ads were his in an interview with the New Yorker:

% I’ve got good news for you: the New Yorker article in question is based on literally one guy on Twitter wanting to teach a shorter version of the case. It’s a completely manufactured fake controversy

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \begin{table}
% \centering% This is an environment - we probably don't want the extra spacing of center in addition to that added by table etc.
% \caption{``Utilidad y Derivación de las Emociones Primarias (Riso, W., 2008)''}

% \small
% \begin{tabular}{*{2}{p{.425\linewidth}}}% The target layout does not centre the text so we don't want \centering
%   \toprule% nicer rules courtesy of booktabs - but then we need to drop the verticals 
%   Emociones primarias &  Derivación de las emociones primarias \\\midrule% Note that there is no & before the first column - & only comes between columns so if you define n columns, you can have at most n-1 & symbols in any row
%   \textbf{Dolor} & \textbf{Sufrimiento}% No need for 6 rows of space for each title!
%   Avisa cuando un órgano físico está funcionando mal o está siendo agredido, para que sea reparado o defendido. & Indica que hay una estructura mental afectada o un apego irracional que debe ser trabajado.\\\midrule% the p{} setting automatically lets these be multi-line - we don't want multiple rows on top of that and this is simpler as TeX does the hard work for us
%   \textbf{Miedo} & \textbf{Miedo psicológico}\\
%   Protege ante un peligro real.& Indica que se ha dejado de actuar. La parálisis es sostenida por ideas irracionales.\\
%   \bottomrule
% \end{tabular}
% \end{table}
\newpage

% \haoran{need elaboration and examples}
% \haoran{why label description can have minor change?}
% researchers tend to change label discription in order to get better performance.
% However, \cite{liu2021gpt} find that the LMs performance are very sensitive to a minor change in label description. the task reformulation methods fully rely on the LMs to understand the label descriptions. 
% \haoran{need elaboration} 
% Furthermore, labeled exemplars provide rich information about the labels and linguistics knowledge.
% However, all of them focus on the few-shot setting and underuse megabytes of labeled exemplars in the fully supervised setting. 
% Moreover, unsupervised contrastive learning has already shown its potential to 


% \haoran{ongoing...}
% \haoran{need running example?}
% In this paper, we aims to solve the problem of the universal NLP classification in the fully supervised setting by leveraging all the existing labeled data by supervised contrastive learning. 
% Our assumption is that the human knowledge is more than label description and hidden in the sentence pair comparison. 

% \haoran{exp: a. f(q, c, h) gt f(q, h) b. f(q, c\_random, h) gt f(q, c\_picked, h), c. interpretabilities of f(q, c, h) and f(q, h)}

% our edges are on three sides:

% \begin{itemize}
%     \item we proposed a unified framework for universal NLP classification for both few-shot setting and fully supervised setting.
%     \item Our method emphasize on text comparison with the labeled exemplar, which provides better interpretability and  lower dependency on label descriptions than the prompt /\ cloze based methods.
%     \item Our method can further boost the performance of finetuning in fully supervised setting by picking the most contrastive exemplars. 
% \end{itemize}




% \begin{enumerate}
%     \item lm-fine-tune -> lm as few-shot learner => mine the knowledge hidden in the unlabeled data
%     \item the large-scaled existing annotated data is under-exploited -> but they cannot be fitted in the contrastive learning framework (pet) due to the ambiguity of natural language classification.
%     \item we propose a unified framework for nlp classification task, entailment of entailment, and show that every classification task can be re-formulated to this form, thus enabling large-scaled training on labeled data.
% \end{enumerate}



% % \begin{enumerate}
% %     \item Why F(q, c, h) is better than the entailment of query and label description F(q, h)?
% %     \item Why F(q, c, h) is better than the pairwise contrastive learning F(q, c)?
% % \end{enumerate}

% % \begin{enumerate}
% %     \item F(q, h) cannot fit in the contrastive learning framework, which has shown its effectiveness in recent self-supervised learning work. sensitive to prompt or cloze question. Experiments are necessary.
% %     \item F(q, c) in NLP classification is ambiguous. In SSL of CV and NLP, an instance is similar with its own data augmentation and dissimilar with other instances. NLP classification is more complicated than this scenario. We can ask different questions to one query sentence, and the contrastive label to other sentence also relies on the question, e.g., F(q, c, h1) != F(q, c, h2)
% % \end{enumerate}

% prompt-based \ cloze question based few-shot learner is sensitive to the human-curated templates \cite{gao2020making}. They still rely on the unsupervised LM to understand the labels through label descriptions. 


% supervised contrastive learning in NLP could be ambiguous as we can ask different questions \cite{schick-schutze-2021-exploiting}


% entailment reformulation is able to conduct zero-shot learning, however, we cannot further boost the performance by feeding related data into the model.

why f(q, c, h) is better than f(q, h)?


suppose 

    g(s1, a) == 1
    g(s2, b) == 1
    g(s3, c) == 0
    
Entailment as few-shot learner:

    f(s1, h\_a) == 1
    f(s2, h\_a) == 1
    f(s3, h\_a) == 0
    
    
you still rely LMs to fully understand label descriptions and learn to extract the related features from several training sentences, although it's easier than by label name only.

Entailment of entailment

    f(s1, s2, h\_a) == 1
    f(s2, s1, h\_a) == 1
    f(s3, s1, h\_a) == 1
    f(s3, s2, h\_a) == 0

the model should focus on the similarity and difference of sentence pairs and match the pair feature to the label description. I think this task definition is easier than entailment as few-shot learner. 

Thus, to further boost the performance of an existing entailment of entailment model, instead of struggling on designing better description of labels for a black box, we can focus on picking more contrastive exemplars.  




better interpretability 
% https://arxiv.org/pdf/1703.01365.pdf
% https://github.com/cdpierse/transformers-interpret

==> deprecated_one_shot_intro.tex <==
% \section{Outline}
% \begin{quote}
    
%     The well-studied within-dataset FSL is not true FSL, then
    
%     True FSL was mission impossible before pretrained LM evolves. Although recent papers of LM few shot learner are the closest to true FSL, no one gives a clear definition, then
    
%     Our paper is the first one that defines true FSL formally as Cross Dataset Few Shot Learning, then
    
%     CDFSL is so true that NLPers have been longing for decades. E.g. We only have an annotation guideline for DARPA evaluation. To pass the evaluation, since there is no true FSL model, we have to collect training data from the web by ourselves and to hire annotators trained by the guideline. If we have a CDFSL model, we can directly apply it to the annotation guideline and pass the evaluation in one hour. And I believe this challenge happens in the industry every day.
    
%     Existing LM few shot learners are the closest to solve this problem, but they miss some important things in CDFSL, then
    
%     1. They did not make full use of all existing labeled data for supervised pretraining. Considering the real-world usage, this should be allowed.
%     2. They still need at least 8 examples per label for training in the target dataset (N-way-8-shot). However, even in the within-dataset "fake" FSL, models can be evaluated by N-way-1-shot.
    
%     , then
    
%     We set up the benchmark of CDFSL, and propose the first valid baseline model for this task. [use a figure to explain entailment of entailment].
    
%     , then
    
%     Our contributions:
%     1. We are the first to introduce CDFSL task formally.
%     2. Like pretrained LM is the first to bridge all the unlabeled data, our model is the first to bridge all the labeled data.
%     3. We set up the CDFSL benchmark and propose the first valid baseline model in CDFSL, which can be evaluated in N-way-K-shot (K > 0) setting.
% \end{quote}

\section{Introduction}
\begin{enumerate}
    \item universal classification task definition
    \item generative style vs kNN style for universal classification
    \item we propose a better supervised pretraining strategy for universal classification.
    \item (exp) how many support examples can help with new task?
\end{enumerate}




% \haoran{Need to mention text classification with different parameters.}
Text classification with limited resources has been in great demand by researchers. 
% In the past decades, NLP researchers have set up many benchmarks for this purpose in one of the most widely applied scenarios, Few-Shot Learning (FSL)
In the past decades, one of the most widely applied scenarios, Few-Shot Learning (FSL) \cite{10.5555/3157382.3157504,10.5555/3294996.3295163,pmlr-v70-finn17a}, has been introduced to many NLP areas \cite{blitzer-etal-2007-biographies,gao-etal-2019-fewrel,larson-etal-2019-evaluation,ding-etal-2021-nerd}.
% NLP researchers have set up many benchmarks for this purpose in one of the most widely applied scenarios, Few-Shot Learning (FSL)
FSL model is required to assign one label to the query sentences from $N$ classes with $K$ annotated examples of each ($N$-Way-$K$-Shot FSL). To make the learning process feasible, the datasets additionally provide large meta-training datasets, either in the same domain or for the same task, but with no class overlapping with the meta-test data.


% \haoran{todo: add more prompt bibs}
Recently, universal few-shot learners have been developed from the pretrained language models (PLMs) \cite{NEURIPS2020_1457c0d6,yin2020universal,gao2020making,schick-schutze-2021-exploiting,schick-schutze-2021-just,du2021all,liu2021gpt,wang2021entailment}. The models use prompt-based learning paradigm which integrates isolated classification tasks from various datasets into one unified task. 
By solving the unified task, the prompt models can directly derived the results same as the non-prompt models trained from the isolated tasks.
Comparing with the fully supervised learners, the universal few-shot learners need only 1\% annotated data to achieve comparable performances \cite{le2021many}.
Comparing with the conventional Few-Shot learners, the universal models discard the meta-training set and the development set \cite{perez2021true}, and work even in stricter settings, e.g., cross-domain or cross-task \cite{ye2021crossfit,bragg2021flex}.
% by reformulating the dataset-specific head  
% in different kinds of datasets to task-agnostic prompt, cloze, or entailment question answering. 
% The universal few-shot learners has obtained better generalization in cross-domain, cross-task settings than the conventional models, even without the dependencies on task-specific training or development data. 
% Comparing with the fully supervised setting, the universal few-shot learners need only 1\% annotated data to achieve the same performance \cite{le2021many}.
% \citet{le2021many} have shown that

% Recently, the prompt-based language models gain better performances even in stricter settings than the conventional FSL, some notable cases including:

% \begin{itemize}
%     \item Training and development data are no longer needed. The model can be directly deployed to test data with or without fine-tuning.
%     \item The evaluation could be cross-task or cross-domain, as the model can be viewed as a universal few shot learner. 
% \end{itemize}

% Besides, the new FSL setting also requires some minor additional resources. Label prompts or label definitions are essential to activate the models, and the information of the labels can be easily found in the dataset description or annotation guideline. \aysa{may keep}
% \haoran{1. classification with parameters. 2. K and N. 3. intermediate training.}
  \begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\textwidth]{images/entail2_intro.pdf}
  \caption{
%   \textsc{flashcard} classification for the pre-segmented sentence \textbf{S}. 
    For a new target dataset, a few label definitions and exemplars are all we have, like a pile of flashcards. Our proposed Entail2 model integrate classification with exemplar into the supervised pretraining: if the (\textbf{Q}uery) sentence entails the \textbf{H}ypothesis label with an \textbf{C}ontext exemplar.}
%   To classify a sentence with any numbers of segments of interest (parameters), the model finds the most relevant flashcards: 
%   if the \textbf{S} emphasized by parameters (\textbf{Q}uery), entails the entailment label, that co-defined by the \textbf{P}rimise and the \textbf{H}ypothesis, the query will be classified to the \textbf{L}abel of the primise. The blue card is for 2-parameter relation extraction task and the red card is for 1-parameter aspect-based sentiment analysis.}
  \label{fig:intro}
  \end{figure}
In spite of the great potentials of the new learning paradigm, existing solutions are not as universal as they should be, because they only solve subsets of problems of non-universal FSL. To the best of our knowledge, none of them covers \textit{all} aspects of the true universal FSL:
\begin{itemize}

    \item The conventional FSL settings can be evaluated on very small $K$, for instance, $K$ can be as small as 1 to 5. However, \citet{gao2020neural,wang2021entailment} and \citet{ye2021crossfit} have to take $K$ more than that as the cost of replacing the conventional meta-training with fine-tuning during meta-testing. 
    
    % \item Some prompt-based models are unable to cope with large $N$, as their prompt lengths grow as the class numbers increase \cite{gao2020making,bragg2021flex}. 
    % In reality, Universal FSL is expected to classify all the labels in the target dataset, beyond the constraints of the conventional FSL.
    
    % The number of classes, $N$, is determined by the datasets in the fully supervised setting. 
    % but is assigned manually in the conventional FSL. Universal FSL models can do both, and we argue the former fits the reality more.
    
    
    % \item \haoran{this is doable by modifying the prompts in other baseline. Maybe we should remove this item.}
    % The existing universal Few-Shot Learners only consider sentence classification task \cite{NEURIPS2020_1457c0d6}.
    % % setreat every token in the sentence equally because that's what sentence classification task based on \cite{NEURIPS2020_1457c0d6}. 
    % They should not, because some tasks are more complicated in a way that the results change when they consider different entities.
    % For example, Relation Extraction (RE) makes classification based on given entity pairs and similarly, Aspect-Based Sentiment Analysis (ABSA) is provided with a aspect word.

    \item The existing universal Few-Shot Learners underuse the long-existing annotated datasets from the whole NLP community.
    The generalization of the prompt models highly rely on the understandings of the label descriptions, but they can be hardly mined from the PLMs without a large-scale supervised pretraining.


\aysa{Why do we need entailment of entailment?}
\aysa{What is entailment? example?}
\aysa{example of entailment of entailment.}

    
\end{itemize}

% \haoran{Not yet finished below}

% To satisfy all the desiderata above, we propose a new framework,  which 
% comprehends the label description with exemplar in the inference stage and 
% learn the general label information from supervised intermediate training on all existing labeled dataset.
% \aysa{how is this relevant to solving the problem? elaborate}
% We bridge labeled data from different tasks by reformulating them into a unified \textbf{E}ntailment of \textbf{E}ntailment ($\text{E}^2$) task. 
% \aysa{Why do you suddenly start talking about E2? How does it connect with the previous part?} 
% For a query sentence $Q$, the model is asked whether or not $Q$ entails the exemplar entailment defined by the \text{label hypothesis} $H$ and its corresponding \text{premise} $P$.
% For example, in Fig. \ref{tab:intro}, the model are asked to classify the query sentence $Q_a$ parametered by $Alex Ross$ and $The New Yorker$. The prediction is conducted by answering the question that whether $Q_a$ entails the exemplar entailment defined by $H_1$ and  $P_1$, both parametered by $LindaJ.Bilmes$ and $HarvardUniversity$.

% The new method is good because ...

% The experiment results are good ...



==> project.tex <==
\section{paper list}
\subsection{Writing Reference}
\begin{itemize}
    \item Universal Natural Language Processing with Limited Annotations: Try Few-shot Textual Entailment as a Start \cite{yin2020universal}
    \item CROSSFIT : A Few-shot Learning Challenge for Cross-task Generalization in NLP \cite{ye2021crossfit}
    \item FLEX: Unifying Evaluation for Few-Shot NLP \cite{bragg2021flex}
    \item A Unified Generative Framework for Aspect-Based Sentiment Analysis \cite{yan-etal-2021-unified}
    \item Incremental Few-shot Text Classification with Multi-round New Classes: Formulation, Dataset and System \cite{xia-etal-2021-incremental}
    \item Meta-learning for Few-shot Natural Language Processing: A Survey
    \item Learning to Segment Every Thing
    \item True Few-Shot Learning with Language Models \cite{perez2021true}
    \item How Many Data Points is a Prompt Worth? \cite{le2021many}
    \item Making Pre-trained Language Models Better Few-shot Learners \cite{gao2020making} \haoran{This method is not capable of classifying many classes.}
    \item Entailment as Few-Shot Learner \cite{wang2021entailment}
    \item Exploiting Cloze-Questions for Few-Shot Text Classification and Natural Language Inference \cite{schick-schutze-2021-exploiting}
\end{itemize}

\subsection{Exemplar theory}

\begin{itemize}
    \item google search "exemplar linguistics"
    \item Prototype and Exemplar-Based Information in Natural Language Categories \footnote{\url{https://ppw.kuleuven.be/okp/_pdf/Storms2000PAEBI.pdf}}
\end{itemize}

\subsection{Few-Shot Learning by Task Reformulation}
\begin{itemize}
    \item GENERALIZATION THROUGH MEMORIZATION: NEAREST NEIGHBOR LANGUAGE MODELS
    \item IEPT: INSTANCE-LEVEL AND EPISODE-LEVEL PRETEXT TASKS FOR FEW-SHOT LEARNING
    \item Incremental Few-shot Text Classification with Multi-round New Classes: Formulation, Dataset and System \cite{xia-etal-2021-incremental}
    \item Discriminative Nearest Neighbor Few-Shot Intent Detection
by Transferring Natural Language Inference
    \item True Few-Shot Learning with Language Models \cite{perez2021true}
    \item How Many Data Points is a Prompt Worth? \cite{le2021many}
    \item Unilmv2: Pseudo-masked language models for unified language model pre-training. \cite{DBLP:conf/icml/Bao0WW0L0GP0H20}
    \item Unified Language Model Pre-training for
Natural Language Understanding and Generation \cite{DBLP:conf/nips/00040WWLWGZH19}
    \item It{'}s Not Just Size That Matters: Small Language Models Are Also Few-Shot Learners \cite{schick-schutze-2021-just}
    \item Exploiting Cloze-Questions for Few-Shot Text Classification and Natural Language Inference \cite{schick-schutze-2021-exploiting}
    \item Making Pre-trained Language Models Better Few-shot Learners \cite{gao2020making} \haoran{This method is not capable of classifying many classes.}
    \item Entailment as Few-Shot Learner \cite{wang2021entailment}
    \item Language Models are Few-Shot Learners \cite{NEURIPS2020_1457c0d6} \haoran{This leads the trend of "language model can do anything with a proper prompt."}
    \item Zero-Shot Entity Linking by Reading Entity Descriptions \cite{logeswaran2019zero}
    \item Learning from Task Descriptions \cite{weller2020learning}
    \item Zero-shot Relation Classification as Textual Entailment \cite{obamuyide2018zero}
    \item Collecting Diverse Natural Language Inference Problems for Sentence Representation Evaluation \cite{poliak2018collecting}
    \item Universal Natural Language Processing with Limited Annotations: Try Few-shot Textual Entailment as a Start \cite{yin2020universal}
    \item Benchmarking Zero-shot Text Classification: Datasets, Evaluation and Entailment Approach \cite{yin2019benchmarking}
    \item All NLP Tasks Are Generation Tasks: A General Pretraining Framework \cite{du2021all}
    \item GPT Understands, Too \cite{liu2021gpt}
    \item Ranking Generated Summaries by Correctness: An Interesting but Challenging Application for Natural Language Inference \cite{falke2019ranking} \haoran{This introduces a series of work about sentence pair alignment: whether or not the two sentences contain the same specific information. Methods: a. NLI. b. IE c. QA.}
    \item Document-Level Event Argument Extraction by Conditional Generation \cite{li2021document}
    \item Self-supervised Contrastive Zero to Few-shot Learning from Small, Long-tailed Text data \cite{rethmeier2020long}
    \item Zero-Shot Relation Extraction via Reading Comprehension \cite{levy2017zero}
    \item Entity-Relation Extraction as Multi-Turn Question Answering \cite{li2019entity}
    \item Event Extraction as Multi-turn Question Answering \cite{li2020event}
    \item event extraction by answering (almost) natural questions \cite{du2020event}


\end{itemize}

\subsection{Contrastive Learning \& Loss}
\begin{itemize}
    \item Supervised Contrastive Learning \cite{khosla2020supervised}
    \item Multi-class Classification without Multi-class Labels \cite{mcl19}
    \item SimCSE: Simple Contrastive Learning of Sentence Embeddings \cite{gao2021simcse}
\end{itemize}

\subsection{dataset}
\begin{itemize}
    \item FEW-NERD: A Few-shot Named Entity Recognition Dataset \cite{ding-etal-2021-nerd}
    \item Meta-learning for Few-shot Natural Language Processing: A Survey
    \item FewRel 2.0: Towards More Challenging Few-Shot Relation Classification \cite{gao-etal-2019-fewrel}
    \item one-shot learning for language modelling \cite{ucar2020one} \haoran{this paper is very interesting! It provides method that can transform unsupervised corpus to few-shot learning data. We can boost the performance of other tasks by setting the label words (from other tasks) to the few-shot language model targets.}
    \item wordnet
    \item blue\_benchmark\footnote{\url{https://github.com/ncbi-nlp/BLUE_Benchmark}}
    \item coronabert \footnote{\url{https://huggingface.co/jakelever/coronabert}}
\end{itemize}

\subsection{Videos}
\begin{itemize}
    \item Hinrich Schütze -- ELLIS NLP Workshop - YouTube \footnote{\url{www.youtube.com/watch?v=_YOaRLQnBjc}}
\end{itemize}



==> review.tex <==
\section{Review}

\subsection{Haoran}

\begin{enumerate}
    \item Why F(q, c, h) is better than the entailment of query and label description F(q, h)?
    \item Why F(q, c, h) is better than the pairwise contrastive learning F(q, c)?
\end{enumerate}

\begin{enumerate}
    \item F(q, h) cannot fit in the contrastive learning framework, which has shown its effectiveness in recent self-supervised learning work. Experiments are necessary.
    \item F(q, c) in NLP classification is ambiguous. In SSL of CV and NLP, an instance is similar with its own data augmentation and dissimilar with other instances. NLP classification is more complicated than this scenario. We can ask different questions to one query sentence, and the contrastive label to other sentence also relies on the question, e.g., F(q, c, h1) != F(q, c, h2)
\end{enumerate}

==> tasks.tex <==
\section{Problem Formulation}
Few-Shot Learning is defined as a $N$-Way-$K$-Shot classification task. The task aims to obtain a classification function:
\begin{align*}
f \colon \mathcal{X}, \mathcal{T} &\to \mathcal{Y} \\
x, t &\mapsto y
\end{align*}
\begin{equation*}
    t =
\begin{bmatrix}
y_1     & s_{11} & s_{12} & \cdots & s_{1K}\\
y_2     & s_{21} & s_{22} & \cdots & s_{2K}\\
\vdots  & \vdots & \ddots & \vdots & \cdots\\
y_n & s_{N1} & s_{N2} & \cdots & s_{NK}\\
\end{bmatrix}
\end{equation*}
where $x \in \mathcal{X}$ is the query sentence, $t \in \mathcal{T}$ is the support set of each query sentence , $E$ is the number of classification iterations of the whole dataset, called episodes, and $E =|\mathcal{X}|$,
$y \in \mathcal{Y}$ is the query sentence label. $\mathcal{X}$, $\mathcal{T}$ and $\mathcal{Y}$ are the set contained query sentences, support set of query sentence, and query sentence label, respectively.
The support set $t$ contains $N$ labeled examples of $K$ classes. 
% Each classification iteration of $x$ is called an episode,
% with $N \times K$ annotated examples visible in the support set $\mathcal{S}$.


% $\mathcal{T}$ contains all visible annotated exemplar sentences $\mathcal{S}$ and the label set $\mathcal{Y}$.

\subsection{Conventional Few-Shot Learning}
% \haoran{what about optimization-based models? e.g. MAML}
\noindent \textbf{Resource}: The conventional FSL task divides the whole dataset into three subsets: $\mathcal{D}_{train}$, $\mathcal{D}_{val}$ and $\mathcal{D}_{test}$, namely, meta-training set, meta-validation set and meta-test set. The three subsets have \textbf{no class overlapping} and are \textbf{either in the same domain or for the same task}, in order to keep i.i.d. in the episode-level.
The FSL models are trained in $\mathcal{D}_{train}$. The hyperparameters are tuned by $\mathcal{D}_{val}$ then tested by $\mathcal{D}_{test}$. $\mathcal{D}_{val}$ is about the same size as  $\mathcal{D}_{test}$
In fact, as the annotation difficulty grows as the class number increases, for each subset, the conventional FSL usually reuse the annotated examples to scale-up the episode number $E$, by sampling a large number of support sets from a small number of label set. 

\noindent \textbf{Evaluation}: $\mathcal{D}_{test}$ uses fixed sampled episodes for evaluation. To measure the model generalization with different sizes of resources, the FSL benchmarks usually sample multiple meta-test sets in different $N$-Way-$K$-Shot settings, e.g., $10$-Way-$5$-Shot. 
The evaluation metrics calculate precision on all episodes in $\mathcal{D}_{test}$. 
Although the sampled $\mathcal{D}_{test}$ can be restored to fully supervised setting, the conventional FSL models are not supposed to be compared with the fully supervised models, because the restoring process brings bigger training data and make the comparison unfair.

\subsection{Universal Few-Shot Learning}
% \haoran{todo}

% \haoran{the definitions of support set in the two setting are different ...}

\noindent \textbf{Resource} The universal FSL task aims to work in an extreme low-resource setting. The task deprecates the large $\mathcal{D}_{train}$ and only uses the support set $t$ in $\mathcal{D}_{test}$ for classification, either with or without fine-tuning the models. 
As the universal models are usually compatible with different types of classification tasks, extra resources other than the target dataset can be used for supervised pretraining (intermediate training).
During the learning process in the target dataset, every query sentence $x \in \mathcal{X}$ looks into the same support set $t$ in $\mathcal{D}_{test}$, which means $t$ is the only element in $\mathcal{T}$.
If fine-tuning is included in the learning process, a small $\mathcal{D}_{val}$ can be used for model selection. $\mathcal{D}_{val}$ is about the same size of $t$.




\noindent \textbf{Evaluation}: 
No episode sampling is included in the construction of  $\mathcal{D}_{test}$, as all the episodes use the same support set $t$. 
The shared support set $t$ is basically equivalent with the training set in fully supervised learning - just the size is much smaller. 
Thus, there can be a direct comparison between the universal models and the fully supervised models, and they can use F1 score for evaluation.
In $N$-Way-$K$-Shot setting, $N$ is the size of the label set in $\mathcal{D}_{test}$, which is determined by the dataset. The shot number $K \in [1, 32]$. When $K \leq 8$, the limited number of training examples are not enough for fine-tuning.

